Effective resistance in metric spaces

Effective resistance (ER) is an attractive way to interrogate the structure of graphs. It is an alternative to computing the eigenvectors of the graph Laplacian. One attractive application of ER is to point clouds, i.e. graphs whose vertices correspond to IID samples from a distribution over a metric space. Unfortunately, it was shown that the ER between any two points converges to a trivial quantity that holds no information about the graph's structure as the size of the sample increases to infinity. In this study, we show that this trivial solution can be circumvented by considering a region-based ER between pairs of small regions rather than pairs of points and by scaling the edge weights appropriately with respect to the underlying density in each region. By keeping the regions fixed, we show analytically that the region-based ER converges to a non-trivial limit as the number of points increases to infinity. Namely the ER on a metric space. We support our theoretical findings with numerical experiments.

==> Preamble/BiblioStyle.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% bibliography style      %
\bibliographystyle{unsrt} %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tables/Table1/Table1.tex <==
\begin{table}[htb!]
\caption{Comparison of \methodE, \lapkrr and \falkon for the target in Eq. \eqref{eq:varsinus_target}. For each level $l$ we show the number of landmarks, the mean square error (MSE), and the accumulated time to train the prediction model (Time). 
In parenthesis, in the time column of the \falkon row, is the time to find the optimal bandwidth through cross-validation.}
\tabcap
\begin{center}
\begin{tabular}{c|c|c|c|c}
    & Level &  \# Landmarks & MSE & Time \\ \hline
    \multirow{4}{*}[+0.5mm]{\method} & 5 & \SI{47}{} & \SI{2.55e-1}{} & \SI{77}{\second} \\ 
    & 10 & \SI{392}{} & \SI{3.69e-2}{} & \SI{116}{\second} \\ 
    & 15 & \SI{1525}{} & \SI{8.63e-6}{} & \SI{497}{\second} \\ 
    & 16 & \SI{2302}{} & \SI{6.18e-6}{} & \SI{1194}{\second} \\ \hline
    \multirow{4}{*}[-2mm]{\begin{tabular}{@{}c@{}}\lapkrr (1) \\ $n_l =\SI{1.1e5}{}$ \end{tabular}} & 5 & \SI{1483}{} & \SI{2.56e-1}{} & \SI{143}{\second} \\ 
    & 10 & \SI{1483}{} & \SI{3.65e-2}{} & \SI{413}{\second} \\ 
    & 15 & \SI{1483}{} & \SI{8.72e-6}{} & \SI{825}{\second} \\ 
    & 16 & \SI{1483}{} & \SI{6.85e-6}{} & \SI{922}{\second} \\ 
    & 18 & \SI{1483}{} & \SI{6.55e-6}{} & \SI{1136}{\second} \\ \hline
    \multirow{4}{*}[+1.5mm]{\begin{tabular}{@{}c@{}}\lapkrr (2) \\ $n_l =\SI{2.2e6}{}$ \end{tabular}} & 5 & \SI{1483}{} & \SI{2.56e-1}{} & \SI{2963}{\second} \\ 
    & 10 & \SI{1483}{} & \SI{3.64e-2}{} & \SI{8704}{\second} \\ 
    & 18 & \SI{1483}{} & \SI{8.91e-6}{} & \SI{23113}{\second} \\ \hline
    \methodE & -- & \SI{14830}{} & \SI{5.7e-3}{} & \SI{4642}{\second}+(\SI{27930}{\second})
\end{tabular}
\end{center}
\label{table:compare_falkon_mrfalkon_streamrak_on_varsinus}
\end{table}

==> Tables/Table2/Table2.tex <==
\begin{table}[htb!]
\caption{Comparison of \methodE, \lapkrrE, and \falkon predictions of the target function in Eq. \eqref{eq:dumbell_target}. For each level $l$ we show the number of landmarks, the mean square error (MSE), and the accumulated time to train the prediction model (Time). In parenthesis, in the time column of the \falkon row, is the time to find the optimal bandwidth through cross-validation.}
\begin{center}
\tabcap
\begin{tabular}{c|c|c|c|c}
    & Level &  \# Landmarks & MSE & Time \\ \hline
    \multirow{4}{*}[-2mm]{\method}& 4 & \SI{352}{} & \SI{1.29e-3}{} & \SI{64}{\second} \\ 
    & 5 & \SI{2667}{} & \SI{1.27e-3}{} & \SI{1398}{\second} \\ 
    & 6 & \SI{1858}{} & \SI{8.31e-4}{} & \SI{1462}{\second} \\ 
    & 8 & \SI{1329}{} & \SI{2.75e-5}{} & \SI{2307}{\second} \\ \hline
    \multirow{4}{*}[-3mm]{\begin{tabular}{@{}c@{}}\lapkrr (1) \\ $n_l =\SI{1.8e5}{}$ \end{tabular}}& 4 & \SI{1375}{} & \SI{1.28e-3}{} & \SI{386}{\second} \\ 
    & 5 & \SI{1375}{} & \SI{1.26e-3}{} & \SI{520}{\second} \\ 
    & 6 & \SI{1375}{} & \SI{9.10e-4}{} & \SI{671}{\second} \\ 
    & 8 & \SI{1375}{} & \SI{3.30e-4}{} & \SI{1064}{\second} \\ 
    & 9 & \SI{1375}{} & \SI{3.10e-4}{} & \SI{1287}{\second} \\ \hline
    \multirow{4}{*}[-3mm]{\begin{tabular}{@{}c@{}}\lapkrr (2) \\ $n_l =\SI{1.9e6}{}$ \end{tabular}}& 4 & \SI{1375}{} & \SI{1.34e-3}{} & \SI{4160}{\second} \\ 
    & 5 & \SI{1375}{} & \SI{1.30e-3}{} & \SI{5570}{\second} \\ 
    & 6 & \SI{1375}{} & \SI{9.44e-4}{} & \SI{7168}{\second} \\ 
    & 8 & \SI{1375}{} & \SI{3.16e-4}{} & \SI{11125}{\second} \\ 
    & 9 & \SI{1375}{} & \SI{3.01e-4}{} & \SI{13334}{\second} \\ \hline
    FALKON & -- & \SI{14830}{} & \SI{6.8e-4}{} & \SI{6590}{\second}+(\SI{37561}{\second})
\end{tabular}
\end{center}
\label{table:dumbell_experiment_complexSinus}
\end{table}


==> Tables/Table3/Table3.tex <==
\begin{table}[htb!]
\caption{Comparison of \methodE, \lapkrrE, and \falkon for the low energy system. For each level $l$ we show the number of landmarks, the MSE at step T=50, and the accumulated time to train the prediction model (Time). In parenthesis, in the time column of the \falkon row, is the time to find the optimal bandwidth through cross-validation.}
\tabcap
\begin{center}
\begin{tabular}{c|c|c|c|c}
    & Level &  \# Landmarks & MSE(T=50) & Time \\ \hline
    \multirow{4}{*}{\method} & 2 & \SI{1}{} & \SI{1.12e-1}{} & \SI{31}{\second}\\
    & 5 & \SI{66}{} & \SI{3.39e-5}{} & \SI{498}{\second} \\ 
    & 7 & \SI{659}{} & \SI{1.44e-6}{} & \SI{534}{\second} \\ 
    & 9 & \SI{4085}{} & \SI{3.01e-7}{} & \SI{812}{\second} \\ \hline
    \multirow{4}{*}{\lapkrr} & 2 & \SI{1979}{} & \SI{5.93e-2}{} & \SI{490}{\second}\\
    & 5 & \SI{1979}{} & \SI{2.73e-5}{} & \SI{1463}{\second} \\ 
    & 7 & \SI{1979}{} & \SI{2.16e-7}{} & \SI{2395}{\second} \\
    & 9 & \SI{1979}{} & \SI{1.16e-8}{} & \SI{3550}{\second} \\ \hline
    FALKON & -- & \SI{19790}{} & \SI{5e6}{} & \SI{2934}{\second}+(\SI{1498}{\second})
\end{tabular}
\end{center}
\label{table:doublePend_falkon_vs_streamrak_lowE}
\end{table}


==> Tables/Table4/Table4.tex <==
\begin{table}[t!]
\caption{Comparison of the \methodE, \lapkrrE, and \falkon for the high energy system. For each level $l$ we show the number of landmarks, the MSE at step T=50, and the accumulated time to train the prediction model (Time). In parenthesis, in the time column of the \falkon row, is the time to find the optimal bandwidth through cross-validation.}
\tabcap
\begin{center}
\begin{tabular}{c|c|c|c|c}
    & Level &  \# Landmarks & MSE(T=50) & Time \\ \hline
    \multirow{4}{*}[2mm]{\method} & 2 & \SI{1}{} & \SI{2.70e-1}{} & \SI{49}{\second}\\
    & 5 & \SI{1106}{} & \SI{8.53e-3}{} & \SI{915}{\second} \\ 
    & 7 & \SI{6376}{} & \SI{2.16e-4}{} & \SI{1999}{\second} \\ \hline
    \multirow{4}{*}[2mm]{\lapkrr} & 2 & \SI{1979}{} & \SI{1.72e-2}{} & \SI{522}{\second}\\
    & 5 & \SI{1979}{} & \SI{5.09e-3}{} & \SI{1474}{\second} \\ 
    & 7 & \SI{1979}{} & \SI{1.39e-4}{} & \SI{2431}{\second} \\ \hline
    \falkon & -- & \SI{19790}{} & \SI{5e6}{} & \SI{23830}{\second}+(\SI{11050}{\second})
\end{tabular}
\end{center}
\label{table:doublePend_falkon_vs_streamrak_highE}
\end{table}
